KOLD: Korean Offensive Language Dataset

Recent directions for offensive language detection are hierarchical modeling, identifying the type and the target of offensive language, and interpretability with offensive span annotation and prediction. These improvements are focused on English and do not transfer well to other languages because of cultural and linguistic differences. In this paper, we present the Korean Offensive Language Dataset (KOLD) comprising 40,429 comments, which are annotated hierarchically with the type and the target of offensive language, accompanied by annotations of the corresponding text spans. We collect the comments from NAVER news and YouTube platform and provide the titles of the articles and videos as the context information for the annotation process. We use these annotated comments as training data for Korean BERT and RoBERTa models and find that they are effective at offensiveness detection, target classification, and target span detection while having room for improvement for target group classification and offensive span detection. We discover that the target group distribution differs drastically from the existing English datasets, and observe that providing the context information improves the model performance in offensiveness detection (+0.3), target classification (+1.5), and target group classification (+13.1). We publicly release the dataset and baseline models.

==> contents/arxiv/0_abstract_arxiv.tex <==
\textit{\textbf{Warning}: this paper contains content that may be offensive or upsetting}

%Although large attention has been paid to the detection of hate speech, most work has been done in English, failing to make it applicable to other languages.
Despite a recent surge in research on hate speech detection, almost all of it is for the few large-resource languages such as English.
%To fill this gap, we present a Korean offensive language dataset (KOLD), 40k comments labeled with offensiveness, target, and targeted group information.
In this paper, we present a Korean offensive language dataset (KOLD), comprising 40k comments on Naver news articles and YouTube videos. 
We label each comment in a hierarchical order: 1) discriminating the offensiveness, 2) categorizing the target of offense, and 3) identifying the specific group if the comment is offensive towards a group of people.
We also collect two types of text spans, offensive spans and target spans, that can justify the classification offensiveness and target type. 
We publicly release the dataset and models trained with our dataset. 
We employ a multi-task learning approach to train a model that 
classifies the comment and provides rationales for the decision.
Comparing the distribution of targeted groups with the existing English dataset, we point out the necessity of a hate speech dataset tailored for the language that best reflects the culture.
We also show that the title of the article and video serves as context, assisting the model in discerning the target of hatred, especially when they are omitted in the comment.
%Comparing the distribution of targeted groups with the existing English dataset, we point out the necessity of a hate speech dataset fitted to the language that best reflects the culture. 

%Comparing the distribution of targeted groups with the existing English dataset, we point out the necessity of a hate speech dataset fitted to the language that best reflects the culture.
% Trained with our dataset, we report the baseline performance of the models built on top of large pretrained language models. 
% The benchmark is further annotated with offensive clauses and target mentions within the sentence, and the title information is given as context where the comment is posted on. 

% The pervasiveness of offensive languages on social media is a widespread phenomenon across the culture. -> 별로인 문장 

% We compare the distribution of target groups with dataset in English and point out the necessity of hate speech dataset that best reflects its culture.

% offensive clause 라는 표현으로 대체
% annotated with corresponding offensive span, target of hate speech, and mentions of these target within the text. 
% The benchmark is specifically annotated with fine-grained target groups and their corresponding target spans, and show that models trained with the dataset can detect newly coined hate-terms. 

%% v2: 0523
% Despite large attention has been paid in detection of hate speech, most work has been done in English
% , failing to make it applicable to other languages.
% To fill this gap, we present KOLD, Korean offensive language dataset labeled with target and span information.
% Comparing the distribution of targeted groups with existing English dataset, we point out the necessity of hate speech dataset that best reflects the culture. 

==> contents/arxiv/1_introduction_arxiv.tex <==
\input{contents/tables/examples_dataset_v2}

Online hate speech is a growing societal issue. An accurate hate speech detection system can help identifying problematic content as well as the victims of hate speech and the damage they receive \citep{vidgen2020directions}. 
%There have been growing efforts in Natural Language Processing community to develop a robust automatic hate speech detection system. 
To train an accurate system, researchers have studied from taxonomies of hate speech \cite{waseem-etal-2017-understanding, zampieri-etal-2019-predicting} to specific aspects of hate speech, such as strength, types, intentions, targeted communities of abuse, and explainability \citep{davidson2017automated, ousidhoum-etal-2019-multilingual, sap-etal-2020-social, elsherief-etal-2021-latent, mathew2020hatexplain, pavlopoulos-etal-2022-detection}.  
% implicit hate speech \cite{elsherief-etal-2021-latent}, and explainability  \cite{mathew2020hatexplain, pavlopoulos-etal-2022-detection}. %\citet{elsherief-etal-2021-latent} address the issue of implicit hate speech, and \citet{mathew2020hatexplain, pavlopoulos-etal-2022-detection} incorporate the concept of rationales for explainability. 
%Recent works have begun to focus on various aspects of hate speech, such as the strength, types, intentions, and targeted communities of abuse \citep{davidson2017automated, ousidhoum-etal-2019-multilingual, sap-etal-2020-social, elsherief-etal-2021-latent}. 
% Recently, researchers are looking at more specific aspects of hate speech, such as strength, types, intentions, and targeted communities of abuse \citep{davidson2017automated, ousidhoum-etal-2019-multilingual, sap-etal-2020-social, elsherief-etal-2021-latent}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{images/example.jpeg}
    \caption{A translated example of KOLD. The title of the article/video is given during the annotation process to provide context. Along with categorical labels, annotators are asked to mark which part of the sentence justifies their decision.}
    \label{fig:example}
\end{figure}

% However, such exploration was mainly done in English, and datasets in other languages \citep{mubarak-etal-2017-abusive, fortuna-etal-2019-hierarchically, chiril-etal-2020-annotated, rizwan-etal-2020-hate} remain scarce.
Even though hate speech is inseparable from cultural and linguistic attributes behind the language \cite{reichelmann-2021-hate-knows, albadi2018they, ousidhoum-etal-2019-multilingual}, non-English datasets \citep{mubarak-etal-2017-abusive, fortuna-etal-2019-hierarchically, chiril-etal-2020-annotated, rizwan-etal-2020-hate} remain scarce, limiting the development of hate speech detection in other languages.
% The focus of hatred differs between cultures \citep{reichelmann-2021-hate-knows}. 
% For example, \citet{ousidhoum-etal-2019-multilingual} observe significant differences in target attributes and target groups of the three languages (English, French, and Arabic).  
% Moreover, hateful comments online often exhibit textual variants such as incorrect grammar, typos, slang, abbreviations, and text containing multi-lingual scripts \cite{albadi2018they} to avoid surveillance. Translating the text cannot convey these elements, which is why dataset fitted for each language is necessary.  
Although there are existing publicly available Korean hate speech corpora \citep{moon-etal-2020-beep, kang2022korean}, our dataset is bigger in size, focuses on more diverse aspects of hate speech and includes span-based annotation.
% For Korean, there are some existing hate speech corpora \citep{moon-etal-2020-beep, kang2022korean},
% they both lack fine-grained categorization of a specific target group of the speech.

To this end, we present an extensive Korean Offensive Language Dataset (KOLD), annotated with 40k comments collected from news articles and videos. 
We add 27 fine-grained target group labels on top of the hierarchical annotation schema proposed by \citet{zampieri-etal-2019-predicting}.
%All annotators are native Korean speakers capable of fully capturing the context behind comments online.
The title of the article and video is given during the annotation process to provide contextual information. 
We also retrieve span-based annotation to identify which part of the sentence makes the given speech toxic (offensive span), or reveals targeted communities (target span). 
To the best of our knowledge, our dataset is the first attempt to annotate both information. 
An example of our data is illustrated in Figure \ref{fig:example}, along with annotation steps.

The main contributions of our work can be summarized as follows:
\begin{itemize}
    \item We present an offensive language dataset in Korean, annotated with target groups fitted to the Korean culture and make it public for future usage.\footnote{available at this \href{http://demos.uilab.kr/demo/Korean-Hate-Speech-Dataset}{link}}
    \item We provide the title as context during the annotation process and show that title information improves performance in target group classification.
    \item We collect span-based annotation of offensive clauses and target mentions in the comment and train models capable of detecting them.  
\end{itemize}


==> contents/arxiv/2_annotation_task_design_arxiv.tex <==
% schema / scheme -> schema 로 통일합니다.

\section{Annotation Task Design}
We use a hierarchical annotation framework split into three levels deciding (1) offensiveness of a comment, (2) a target type of the offensive comment, and (3) a specific target category if the comment is targeted at a group characteristic. First level has two possible answers: \textit{offensive, not offensive}, second has four: \textit{untargeted, individual, group, others}, where a comment is classified as others when it is a targeted offensive speech but the type of the target is neither group nor individual. The third level has 27 possible choices (see Appendix for the full list of target groups). We also collect span annotations that support the labeling decision, if the comment is offensive or contains the target of the offensiveness (see Figure~\ref{fig:example}). 
%For the first two levels, we reuse the definitions suggested in \citet{zampieri-etal-2019-predicting}, which have been adopted in several datasets \citep{zampieri-etal-2020-semeval, zeinert-etal-2021-annotating, rosenthal-etal-2021-solid}.

% If a comment is annotated to be offensive, the next annotation item is the target. This can be either ``none'' (i.e., the comment does not specify a target), or a group, an individual, or ``other'' (e.g., an organization, a situation). If the target is annotated as ``group'', then the next annotation item is the specific target group among 27 possible groups that include women, men, Christians, etc. Please see Table \ref{tab:target_group_dist} for the list of the target groups.

We extend the multi-layer annotation schema in \citet{zampieri-etal-2019-predicting} with an additional step for identifying the specific target group of the comment, so that the trained model can be used to address the harm incurred by the offensive comment, such as social bias \citep{blodgett2020language}.
In addition, we ask the annotators to ground their judgement by marking spans in the text that reveal offensiveness or indicate the target group.
%In the following section, we provide the detailed definitions of the target group and span annotation.

%\textbf{Offensiveness} is the primary goal of the annotation, and is the first category to label. There are two possible answers: offensive or not. Following \citep{zampieri-etal-2019-predicting, zeinert-etal-2021-annotating}, we consider a comment as offensive if it contains any form of untargeted profanity or targeted offense such as insults and threats, which can be implicit or explicit. 

%\textbf{Target} aims to capture the type of the target of the offensiveness. The possible answers are: Group, Individual, Others, Not specified. For group, individual and others, we reuse the values and definitions from \citep{zampieri-etal-2019-predicting}.  

\subsection{Target Group Annotation}

%Target group is a social or demographic group the offensive speech is referring to. Since deciding what should be considered \textit{protected characteristics} is a controversial issue \citep{vidgen2020directions}, we provide a list of potential target groups and their attributes based on all characteristics appeared in the source corpora.

Before main annotation, we define a list of target groups based on social and demographic characteristics. We initially begin with the categorization of targets in \citet{sap-etal-2020-social} and add several categories to better reflect the distribution of Korean data. 
The top level group categories, i.e., Target Attribute, are shown in Table~\ref{tab:distribution}, and the subsequent level group categories are shown in Table~\ref{tab:target_group_dist}.
After analysis of targets of hate speech with 1,000 samples, \textit{Chinese}, \textit{Korean-Chinese}, and \textit{Indian} are introduced to \textit{Race, Ethnicity \& Nationality} category, as they take up a bigger portion than the initial target groups (\textit{White}, \textit{Asian}).
%\textit{Chinese} (3.98\% of the group-targeted comments), \textit{Korean-Chinese} (4.48\%), and \textit{Indian} (1.49\%) are introduced to \textit{Race, Ethnicity \& Nationality} category, as they take up a bigger portion than the initial target groups (\textit{White}, \textit{Asian}).
% Infrequent group characteristics are incorporated under the attribute \textit{Miscellaneous}, as well as those that do not belong to the rest of the categorizations (e.g., Feminists). 
Group characteristics that do not belong to the rest of the categorizations (e.g., \textit{Feminists}) are incorporated under the attribute \textit{Miscellaneous}.
The final categories of target groups and their attributes included in the dataset are listed in Appendix \ref{table:appendix_group}.

%First we start out with following target attributes: Gender, Sexual-orientation, Race, Religion, Political affiliation and Miscellaneous (Misc.). We first start out with target attributes, i.e. protected characteristics, and list the specific target groups that belong to the characteristics. 
%For each attribute, we list the specific target groups of the attributes, resulting in following target groups: women, men, gender-queer (Gender); homosexual, lesbian, gay (Sexual orientation); Black, White, Asian (Race); Christian, Catholic, Buddhist, Islam (Religion); Conservative, Progressive, others (political affiliation); feminism, age, physical appearance, disability, disease, and socioeconomic status (Misc.). We also provide group "others" for each attribute, to label groups that are not listed in our preset.

%After annotation of the first 1,000 comments, we revise the categorization of target groups in a way that better reflects the distribution of the actual data. For example, we add new target groups Chinese (3.98\% of the group-targeted comments), Korean-Chinese (4.48\%), Indian (1.49\%) as they take up bigger portion than existing target groups (White, Asian). We adjust the target attribute accordingly, by expanding the previous "race" category to include ethnicity, nationality as well. We also merge the target groups homosexuals, lesbian, gay, and gender queer into a one target group "LGBTQ+", as well as the corresponding target attributes, due to the confusion shown in the result.  %Table \ref{tab:target_group_dist} shows target groups that frequently appear in each target attribute.

\subsection{Span Annotation} \label{sec:span annotation}
To provide a human explanation of categorization, we collect rationales for the offensiveness and target of hate speech. Following \citet{zaidan2007using}, we define rationale as a specific text segment that justifies the human annotator's decision of the categorization. We ask the annotators to mark the span within the given text if the text is offensive or has specific target.

\paragraph{Offensive span} If the comment is classified as \textit{offensive}, we ask the annotators to highlight a particular span of characters in a comment that supports their judgment about the label. Offensive span does not necessarily exhibit explicit expressions but can convey nuanced, implicitly offensive messages. In order to collect the precise span that is informative about the categorization, we consider two components of \textit{faithfulness}, presented in \citet{deyoung-etal-2020-eraser}: sufficiency and comprehensiveness. We guide the annotators to highlight a minimal span of characters from the text that supports the judgment (sufficiency) while including non-verbal expressions such as emojis and morphemes that are used to convey the intention to assault, insult or demean as well (comprehensiveness). % 예시문장 하나 (nuanced hate speech)

Pinpointing the specific span of offensive remark is essential, as not all sentences or comments that include such span are necessarily offensive. Utilizing the relation between an offensive clause with other elements of the context can facilitate the model to correctly identify implicit and nuanced offense as well \citep{wiegand-etal-2021-implicitly-abusive}. Moreover, the spans may be used to train explainable models, as is shown in recent works \citep{mathew2020hatexplain, lei2016rationalizing}. 

\paragraph{Target span} 
Target span is a span of characters that appear in the comment that indicates the target of the hate speech. 
It is collected for all types of \textit{targeted} offensive speech, regardless of the type of the target (individual, group, or others). 
If the term used to indicate the target itself is offensive, target span overlaps with offensive span (e.g., \textit{jjangkkae}, which corresponds to \textit{ching-chong} in English). 
Distinguishing simple identity terms from hate terms can help address models showing spurious correlation to identity terms reported in many previous works on hate speech \citep{kennedy-etal-2020-contextualizing,dixon2018measuring}. 
%Aspect-based sentiment analysis와 유사한 setup, thus can be used to learn the relationship between the subject and predicate 


==> contents/arxiv/3_collecting_annotations_arxiv.tex <==
\section{Collecting Annotations}

%\textbf{Pilot Annotation}
%During pilot annotation, each annotators are given 100 comments and are asked to perform all three steps of classification tasks. Twelve in-house annotators from a crowd-sourcing company participated. The main purpose of pilot annotation was to check if our guideline was clear enough. The Kripendorff's alpha score for inter-annotator agreement (IAA) are 0.64, 0.55, 0.53 for offensiveness classification, target classification and target group classification respectively. We decide our guideline was clear enough for the classification task, in comparsion to the scores of previous studies. % need stats and ref 

\subsection{Source Corpora Collection}

We choose two social media platforms, Naver and YouTube, as our source of data collection, which are two of the top three mobile apps used in Korea in 2021.\footnote{\href{http://www.koreaherald.com/view.php?ud=20210901001000}{Using big data analysis to chart a new course, The Korea Herald}}
In particular, we collect comments on Naver news articles and YouTube videos distributed from March 2020 to March 2022. 

Due to the scarcity of offensive comments, we collect articles and posts by using predefined keywords, which is a commonly used method in hate speech dataset construction \citep{waseem2016hateful}. Every keyword are potentially highly correlated with articles or videos that may have abusive comments. Keywords listed in in Appendix \ref{appendix:a}.

To remove the users' personally identifiable information, we do not collect user ids. We replace mentions of username in the comment with <user> tokens, URLs with <url> token, and emails with <email> tokens to conceal privacy information.

\subsection{Annotation Process}

We use SelectStar,\footnote{\href{https://selectstar.ai}{https://selectstar.ai}} a crowdsourcing platform in Korea, to collect annotation.
Given a set of comment and title, annotators first decide whether the comment is offensive. 
If the comment is labeled as offensive, the annotators highlight the rationale for such judgment. 
For offensive comments, workers further categorize the target type and highlight the span of characters that indicates the target. 
Finally, if the comment is targeted at a group trait, the specific target group is chosen from our list. 
We allow multi-group annotation if the target entity of the comment belongs to more than one group. 
For instance, ``페미년 (feminist bitch)'', a word that disparages a feminist woman targets two groups: \textit{Gender \& Sexual orientation - Women} and \textit{Misc. - Feminist}. 
We collect three annotations per comment.


Acknowledging the difficulty of acquiring consistent annotation of textual spans, we give specific guidelines for span annotation. \citet{pontiki2016semeval} reports two reasons behind annotator disagreements in span annotations: (i) ambiguity due to lack of context and (ii) multi-word term boundaries. %The former is a salient issue in hate comments since there are many cases where neighboring sentences or context is required for a sentence to be understood as offensive \citep{de2018hate}. Moreover, in Korean, a subject or object is often omitted when can be inferred through context. Thus, contextual information is essential for a reader to decide if a sentence is a targeted offensive speech. 
To deal with the first issue, we make it clear that annotators use the title of the article or video as context. For the second issue, we provide a detailed guideline to satisfy \textit{faithfulness} (see section \ref{sec:span annotation}), and to decide morphological boundaries specific to Korean.

As hate speech annotation can be influenced by the bias of the annotators \citep{davidson-etal-2019-racial, sap2021annotators, al-kuwatly-etal-2020-identifying}, we aim to collect judgement of as diverse annotators as possible. We limit the maximum amount of annotation per person to 1\% of the total data. To ensure annotation quality, we only allow the users who pass a qualification test to proceed to the main annotation process. The test is comprised of 20 categorical questions that have clear answers. To prevent scams during the annotation process, we use fake questions with 40 comments and answers to block users who give wrong answers. A total of 3,124 annotators have participated in creating the final dataset. 

Overall, the average Krippendorff's α for the inter-annotator agreement is 0.55, which is higher than other hate speech datasets with complex annotation schema \citep{mathew2020hatexplain, ousidhoum-etal-2019-multilingual}. Specifically, α is 0.55 for classifying offensiveness, 0.45 for deciding the target type, and 0.65 for specifying the target group of the offensive speech.

To decide on the gold label, we apply majority voting. 
For categorical labels, what more than two out of three annotators choose is selected as gold label. 
For target type selection and target group selection, there are cases where label cannot be determined by majority voting as there are more than two choices.
The inspectors are at the last step to give decision of the final label. 
Inspectors are selected workers who passed the qualification test with higher scores.
In terms of textual spans, characters that are overlapped by more than two annotators are provided as ground truth.

==> contents/arxiv/4_kold_arxiv.tex <==
\section{KOLD: Korean Offensive Language Dataset}
\subsection{Dataset Descriptions}
\input{contents/tables/data_stats}
\input{contents/tables/target_group}

% Average length of the comment in our dataset is 45 characters. 
% Average length of string highlighted as offensive span per post is 22, and that of target span is \~. 
%each categorical label are as follows: offensiveness: 0.55, target: 0.48.  %(계산하는 방식: computed the mean pairwise Kappa per post, by using character offsets as instances being classified in two classes, toxic and non-toxic. And then we averaged Kappa over the total number of posts (SemEval-2021 Task 5: Toxic Spans Detection)) 

% \textbf{Class balance}
The final dataset contains 40,448 comments, of which 20,130 comments are classified as offensive language (Table \ref{tab:distribution}).
%This is comparable to existing datasets for abusive language detection, where the number of abusive samples is much smaller than that of non-problematic samples. 

Offensive speech targeted at group characteristics comprises 31.4\% of the whole data, commonly understood as hate speech \citep{zampieri2019predicting}. 2,596 comments are offensive but not targeted at any particular entity (UNT). Among targeted offenses, group (GRP) is the most common type of target, present in 30.68\% of the whole dataset, followed by individual (IND)(9.64\%) and others (OTH)(3.47\%). Among group-targeted offensive speech, \textit{Gender \& Sexual orientation}, \textit{Race \& Ethnicity \& Nationality} and \textit{Miscellaneous} are the three most common attributes of the target, taking up 7.38\%, 7.34\% and 6.97\% of the whole dataset respectively. \textit{Political Affiliation} and \textit{Religion} both appear less than 5\% of the data.
%Gender \& Sexual Orientation is the attribute targeted most frequently with 2,986 examples, followed by Race, Ethnicity \& Nationality, which is present in 2,970 examples.

\subsection{Target group distribution} 
%The distribution of the target groups in the final dataset reflects the cultural characteristics of hate speech in Korean society. 
Table \ref{tab:target_group_dist} shows a breakdown of target attributes of group-targeted offensive comments in KOLD. We present the statistics for the three most frequent target groups for each target attribute, as well as the group \textit{Others}, which is tagged at the target attribute level but do not belong to the target group choices we provide. The three most frequently targeted group characteristics in the whole dataset are \textit{Feminists}, \textit{LGBTQ+} and \textit{Women}, which amount to 11.42\%, 10.55\% and 8.7\% of the total group-targeted offensive speech, respectively. Target groups in Miscellaneous attribute include groups regarding \textit{Socio-economic status}, \textit{Age}, \textit{Disability}, \textit{Physical appearance}.

The distribution of the target groups for Race, Ethnicity \& Nationality in the final dataset highlights the cultural characteristics of hate speech in Korean society. The two identity groups that appear most frequently as the target of hate speech regarding this attribute are \textit{Chinese} and \textit{Korean-Chinese}. \textit{Others} take up a large portion of this attribute with 1,605 comments, and the specific targeted groups in this category include groups of various origins ranging from Afghans and Americans to North-Koreans and North-Korean defectors. The latter two groups and Korean-Chinese share same ethnicity as Koreans, but their nationality is either China or North Korea. This reflects the reality in Korea, where there exists discrimination of immigrants based on nationality even within Asians who share similar cultural values and phenotype \citep{lee2017neo}.

%\textit{others} is the largest group that belongs to Race \& Ethnicity \& Nationality. The specific targeted groups in this category include groups of various origins such as North-Koreans, North-Korean defectors, Afghans and Americans. However, \textit{Chinese} and \textit{Korean-Chinese} are the two identity groups that appear most frequently as the target of hate speech related to race, ethnicity, and nationality. The targets   This reflects the reality in Korea, where there exists discrimination based on nationality and ethnicity even within Asians who share similar cultural values and phenotype \citep{lee2017neo}.

\input{contents/tables/group_comparison}

Table \ref{tab:hatexplain} compares the distribution of target groups that are present in our dataset and the target communities in the HateXplain dataset \citep{mathew2020hatexplain}. 
We list the top 10 target groups of each dataset based on frequency of appearance.\footnote{We calculate the statistics from the hateXplain dataset ourselves as \citet{mathew2020hatexplain} do not provide the specific distribution of the target groups. We changed the target group \textit{Islam} to \textit{Muslim}, to match with our term.} Interestingly, \textit{Africans}, the target group that appears most frequently in HateXplain, is not included in the top 10 ranked groups in our dataset, and the same is true for \textit{Feminists}, the first-ranked target group in our dataset. Other identity groups such as \textit{Chinese, Korean-Chinese, Progressives} and \textit{Conservatives} only appear in our dataset. While \textit{Women, LGBTQ+} (which includes Homosexual) and \textit{Men} are common target groups in both datasets, we observe that groups such as \textit{Jewish, Arab} and \textit{Hispanic} which commonly appear in existing datasets in English (e.g., \citet{sap-etal-2020-social, ousidhoum-etal-2019-multilingual}), do not appear frequently in our dataset as well. The overall distribution of target groups seems to reflect the cultural difference. 



==> contents/arxiv/5_experiments_arxiv.tex <==
\input{contents/tables/baseline_result}
% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{images/sentence_cls.png}
%     \label{fig:sent}
% \end{figure*}

In this section, we describe the three experiments we take and report the results.
The experiments are (1) sentence classification, (2) span prediction, and (3) ablation of contextual information.
Using a 80-10-10 split for each task, we use various sizes of BERT and RoBERTa pre-trained with Korean~\cite{park2021klue}. 
All experiments are conducted using Transformers library via Hugging Face.\footnote{\href{https://github.com/huggingface/transformers}{https://github.com/huggingface/transformers}}
% Language model are finetuned with the learning rate in \{1e-5, 2e-5, 3e-5, 5e-5\} and the number of epochs in \{1, 2, 3, 4, 5\}\footnote{We kept the batch size fixed at 32 for training, 64 for validation}.
For the experiments, we searched for a learning rate out of \{1e-5, 2e-5, 3e-5, 5e-5\} and the number of epochs out of \{1, 2, 3, 4, 5\}\footnote{We kept the batch size fixed at 32 for training, 64 for validation}.
% We tune hyperparameters on the dev. set, and report the best performance according to F1 score. 
We report the best performance based on F1 Score of dev sets result with tuned hyper-parameters.


\subsection{Sentence Classification}
We employ BERT sequence classification model to predict the (1) offensiveness (binary), (2) target of insult (untargeted, group, individual, others), and (3) 27 fine-grained target groups.
All data is used for offensive classification, data with offensive labels are used for target classification, and group-targeted data is used in group classification sub-task. 
Table~\ref{tab:baseline} shows accuracy and macro-F1 for each sub-tasks.

As the categories are more fine-grained, the task becomes more difficult.
The macro-F1 score of offensiveness classification is above 0.77 in all sizes of the pre-trained language models.
On the other hand, in the fine-grained group with 27 labels, the macro-F1 is scored as less than 0.58.
In all three sub-tasks, BERT-base, RoBERTa-base, and RoBERTa-large perform well in the order.
The larger the model, the better the understanding of hate speech.

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{images/span_cls.png}
%     \label{fig:span}
% \end{figure*}

\subsection{Span Prediction}
We view the span prediction task as token classification task.
We employ BERT token classification model~\cite{wolf-etal-2020-transformers} and convert each span to BIO-tag which is widely used in the Named Entity Recognition (NER) task to  predict if each token corresponds to a span.
By doing this, we can handle spans that appear truncated in the sentence.
After prediction, we post-process token-prediction results to text and compare them with gold span in character level. 

We use Exact Match Accuracy (EM), Rationale F1 (RF1), Intersection Over Union F1(IOU F1) to measure how well the predicted rationale agree with those marked by humans (plausibility).
Exact Match Accuracy (EM) is character-level accuracy, how exactly predictions is matched with gold spans. 
Rationale F1 (RF1)~\cite{da-san-martino-etal-2019-fine, pavlopoulos-etal-2021-semeval} is character-level F1 score.
In detail, it is the f1 score derived by precision and recall which is calculated by counting the matching the number of characters.
Intersection Over Union F1 (IOU F1)~\cite{deyoung-etal-2020-eraser} is also f1 score derived by precision and recall which is calculated as prediction matches more than a certain threshold. Here we use 0.5 as threshold. 

We report the results of the span prediction in the bottom half of Table \ref{tab:baseline}.
All three metrics show the same tendency, a high score in one metric results in a high score in the other two metrics.

Aligned with the result of sentence classification, there is also a tendency according to the size of the model.
In all cases, the model with large capacity outperforms.
% On the other hand, in target span prediction, the larger the model, the lower the performance on all three metrics.
% 생각 하는 이유

% 이 실험은 일단 없어져서 빼야할듯
% Second, we measure how these rationales have meaningfully influenced it's prediction using comprehensiveness and sufficiency. 
\input{contents/tables/ablation_title_headline}
\input{contents/tables/context_analysis}

\subsection{Ablation of Title Information}

We conduct an ablation study by excluding the title from the input to check how much giving the title to model contributes to specifying the context in the comment.
Table~\ref{tab:headline} shows the results of this experiment.
Compared to the case where title comment are given together if only comment is given, accuracy and f1 score drop significantly.
This phenomenon become more significant as the granularity of the label increased.
When predicting the fine-grained target group, the accuracy dropped by 0.22 and f1 score by more than 0.12. 
Table \ref{tab:span} shows the number of comments where offensive and target span are absent.
Sentences that are group targeted but does not have target span in the comment is up to 55\% while offensive posts that does not have offensive span in the sentence is only 9.3\%. 
One of the possible reasons behind this is because Korean is a null subject language \citep{kim-etal-2000-subject}, the mentions of targeted communities is often omitted.  
We conclude that providing title helps model to predict the target group more precisely it is absent in the comment. 

% We use the same BERT token classification model to test how well a model can predict the target span with the unseen terms in data. Since we are only looking at how model accurately predicts the span, we only use plausibility metric from above during evaluation. 

% \textbf{Target Span Prediction Over Time}


==> contents/arxiv/6_related_work_arxiv.tex <==
\section{Related Work}
% The resource with Korean is extremely scarce, having 9.4K labeled corpus with single level annotation of offensiveness and hatred \citep{moon-etal-2020-beep}. 

\subsection{Definition}
%While there is no single definition of hate speech established in the literature, 
% Term \textit{offensiveness}, \textit{toxicity}, and \textit{hate speech} are 
While the definition of hate speech differs among literature, the elements of hate speech can be summarized into the following: 1) demonstrates a clear intention to incite harm, or 2) promote hatred towards individuals or groups based on their characteristics \citep{zhang2019hate, richardson2018woman}. 
%We define the former as offensive texts and the latter as cyberbullying (individual) and hate speech (group).
The previous line of works following \citep{zampieri-etal-2019-predicting} collects these two information with hierarchical annotation schema. 

% \subsection{Target of Hate Speech}
To reduce representational harm \citep{barocas2017problem} caused by an automated system, it is important to identify in what aspect the speech is problematic (i.e., racist, sexist), and to whom such hatred is targeted. 
Unlike the previous line of works that classifies target into coarse-grained categories such as racism or sexism, recent works aim to identify the specific target group or individuals of hate speech \citep{mathew2020hatexplain, sap2020social, shvets2021targets, ousidhoum-etal-2019-multilingual}. 

% However, the Korean hate speech dataset with fine-grained target group information does not exist. 
% \citep{moon-etal-2020-beep} only contains information of gender bias, and categories used in \citep{kang2022korean} is close to coarse-grained categories not the specific demographic comments are referring to. Our work contains both course-grained target attributes such as gender, race, and religion and fine-grained target groups such as Women, LGBTQ+, and Chinese.

% \citet{moon-etal-2020-beep} only retrieved labels of offensiveness and presence of gender bias, and  all comments are collected from entertainment news. \citet{kang2022korean} poses multi-target label scheme but lacks proper taxonomy.

% 그러나 여전히 한국어 hate speech dataset에서는 이런 fine-grained target group을 고려하는 dataset이 존재하지 않는다. \citep{moon-etal-2020-beep}은 bias의 attribute로서 gender, others만을 다루고, \citep{kang2022korean}에서는 hate speech의 target attribute가 무엇인지만을 다룬다. 우리는 여기서 나아가 한국 문화에서 나타나는 specific target group of the hate speech를 직접 annotation한 dataset을 만든다. 
% 문화 및 언어권마다 hate speech의 target group은 다르게 나타나고\citep{reichelmann-2021-hate-knows}, \citep{ousidhoum-etal-2019-multilingual}는 실제로 observe that there are significant differences in terms of target attributes and target groups in the three languages (English, French and Arabic) of which they constructed hate speech datasets. All three languages에서 공통적으로 나타나는 target group 외에도 “other” 카테고리에서 문화권마다 다른 target group이 나타나는 것을 확인했다 (예를 들어, English와 French에서는 political ideologies, Arabic에서는 Kurdish라는 특정 ethnic group). 

\subsection{Context Information}

Context information in hate speech refers to both previous comments in the same thread and preceding sentences of a document where the comment is posted on. Recently, there were attempts to construct data that contains previous comments \citep{vidgen-etal-2021-introducing}. 
% We acknowledge that providing both information will be helpful, but due to the complexity of data or usage and to focus on target group and title gives more contextual information than previous threads, we use the title information as context.
Hate speech corpus annotated with context was initially constructed by \citet{gao-huang-2017-detecting}, where they provide user name, comments in the same thread, and the news article the comment is written on. 
Among these information, title helped the most when neural net models determine offensive posts. 
However, the number of collected comments in this work is relatively small (1.5k), and only 10 news articles were retrieved. 
We overcome this issue by collecting 40k comments from 2543 different news articles and 1157 YouTube videos. In our study we confine the context as being titles of new articles or videos we have collected comments from. 

% \citet{pavlopoulos-etal-2020-toxicity} investigated if context really affects annotators' judgements and if they improve performance in toxicity detection systems. The result shows that providing context does change the polarity of label in 5\% of comments, but the influence of model performance is surprisingly small. 
% In line with this work, we conduct experiments to see if the context influences model decision in offensiveness, target, and target groups. Our experiments reveal that while providing context does not have significant effect to the decision of offensiveness, it does provide hints to whether the comment is targeted towards group, individual, other or not, and in which community the comment is targeted to. 
% Hate speech의 context information은 크게 이전 쓰레드의 (parent) 댓글 정보와 title 및 기사 내용에 대한 정보로 나눌 수 있는데, 이전 댓글 정보를 context로 활용한 연구랑 논문은 이런게 있지만 \citep{vidgen-etal-2021-introducing} (더 찾으면 추가) 우리가 사용하는 context는 title로 한정한다 (여기서이걸 한계로 적어야할지?). 
% title을 context로 활용한 연구로는 \cite{gao-huang-2017-detecting}에서 가장 먼저 뉴스 제목 본문이랑 유저 아이디를 포함한 데이터셋을 만들었고 실험을 통해 offensiveness 판단에 도움이 되는걸 보여줬다. 하지만 데이터셋이 너무 작고 어노테이터가 거의 한명이 다했다. \citep{pavlopoulos-etal-2020-toxicity} 는 이 부분을 지적하면서 title과 이전 댓글들이 실제로 어노테이션 결과에 영향을 미치는지를 실험을 통해 확인헀는데 case study를 통해 context로 인해서 일부(몇퍼 추가) 댓글의 label이 바뀌는 것을 확인한 반면 context가 실제 모델 inference 성능에 미치는 영향은 미미하다는 것을 밝혀냈다. 이 결과와 비슷하게 우리도 title 정보가 offensiveness 판단에는 큰 영향을 미치지 않지만, 우리는 여기서 더 나아가 본 데이터셋을 통해 target 및 group classification 레이블에는 title 정보가 큰 영향을 미치는 것을 확인할 수 있었다. 

% While there are pile of hate speech dataset labeled with offensiveness and target, few of them provide the context information to human annotators during the collection of data. 
% While offensiveness 랑 target 에 대한 연구는 많이 이루어진 것에 비해서 context 정보를 반영한 데이터셋은 많지 않은데,영어로는 이런게 있고\citep{gao-huang-2017-detecting, xenos-etal-2021-context}, 다른 나라 언어로는에서 \cite{mubarak-etal-2017-abusive} 가 유일하게 title 정보를 추가했다. 


\subsection{Explainability of Hate Speech}
Explaining the decisions made by the model is an important step in deterring users from posting harmful comments. Such supporting evidence, also well known as ``rationale,'' can be acquired automatically generated by machines or hand-crafted by human annotators. Techniques to generate rationales by machines were suggested, such as model-agnostic approaches \citep{ribeiro-etal-2016-lime, lundberg-etal-2017-shap}, allocating importance attribution score to each feature \citep{Jin2020Towards}, and in many other methods not listed here. In contrast, human-provided rationales for hate speech are relatively scarce. It was first introduced in \cite{pavlopoulos-etal-2021-semeval} as a toxic span detection task by manually adding toxic spans to the existing hate speech dataset. \cite{mathew2020hatexplain} collected hate speech data from scratch. 

% State-of-the-art models still tend to overgeneralize with slurs or certain identity terms \citep{rottger2020hatecheck, dixon2018measuring}. 최근에는 Hatespeech detection task에서도 model explainability를 평가하기 위해 HateXplain\citep{} benchmark dataset이 등장했다.

% QA, sentiment classification, NLI 등의 task에서 모델의 explainability를 확인하기 위한 데이터셋이 제작되어 왔다\citep{wiegreffe2021teach}.

%\citet{qian-etal-2021-lifelong} : model that adapts to new data without forgetting the previous learned knowledge. 

==> contents/arxiv/ablation_title_arxiv.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule
                                     &                                     & \textbf{$\Delta$ Accuracy}               & \textbf{$\Delta$ F1}                     \\ \hline
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}+ Title\end{tabular}}} & \multirow{2}{*}{\textbf{Offensive}} & \multirow{2}{*}{+1 \small{(1.2\%)}}     & \multirow{2}{*}{+0.2 \small{(0.3\%)}}   \\
                                     &                                     &                                 &                                 \\ \cline{2-4}
                                     &  \multirow{2}{*}{\textbf{Target}}    & \multirow{2}{*}{+1.5 \small{(1.7\%)}}   & \multirow{2}{*}{+2.4 \small{(3.7\%)}}   \\
                                     &                                     &                                 &                                 \\ \cline{2-4}
                                     & \multirow{2}{*}{\textbf{Group}}     & \multirow{2}{*}{+21.6 \small{(38.0\%)}} & \multirow{2}{*}{+13.1 \small{(30.6\%)}} \\
                                     &                                     &                                 &                                 \\ \bottomrule
\end{tabular}
}
\caption{Performance gap in sentence classification task when the title is given. Absolute improvement is reported as +, and percentage gain in parentheses. Overall, model achieves higher scores when the title information is given, and the gap is the largest in group classification task. Pretrained language model is fixed to BERT-base in this experiment.}

\label{tab:headline}
\end{table}

==> contents/tables/baseline_result.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccclcccc}
\toprule
\multirow{2}{*}{\textbf{Task}}                                                              & \multirow{2}{*}{\textbf{Subtask}}        & \multirow{2}{*}{\textbf{\# Labels}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Metrics}}                                                                                                                   \\ \cline{5-8} 
                                                                                            &                                          &                                     & \multicolumn{1}{c}{}                                & \textbf{Accuracy}                     & \textbf{Precision}                     & \textbf{Recall}                    & \textbf{F1}                      \\ \hline
\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sentence\\ Classification\end{tabular}}} & \multirow{3}{*}{\textbf{Offensive}}      & \multirow{3}{*}{2}                  & {\fontfamily{qcr}\selectfont BERT$_{base}$}                                      & 83.9                                  & 75.8                                   & 78.8                               & 77.2                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{base}$}                                   & 81.4                                  & 76.8                                   & 77.6                               & 77.2                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{large}$}                                  & 84.9                                  & 76.6                                   & 81.1                               & \textbf{78.8}                    \\ \cline{2-8} 
                                                                                            & \multirow{3}{*}{\textbf{Target}}         & \multirow{3}{*}{4}                  & {\fontfamily{qcr}\selectfont BERT$_{base}$}                                      & 90.4                                  & 72.6                                   & 68.0                               & 68.0                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{base}$}                                   & 91.3                                  & 71.9                                   & 68.5                               & 70.1                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{large}$}                                  & 92.3                                  & 76.4                                   & 70.7                               & \textbf{72.8}                    \\ \cline{2-8} 
                                                                                            & \multirow{3}{*}{\textbf{Group}}          & \multirow{3}{*}{27}                 & {\fontfamily{qcr}\selectfont BERT$_{base}$}                                      & 78.5                                  & 56.9                                   & 57.4                               & 55.9                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{base}$}                                   & 76.4                                  & 58.6                                   & 58.5                               & 57.3                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{large}$}                                  & 78.1                                  & 59.1                                   & 59.6                               & \textbf{57.5}                    \\ \hline
\multicolumn{1}{l}{\multirow{2}{*}{}}                                                       & \multicolumn{1}{l}{\multirow{2}{*}{}}    & \multirow{2}{*}{\textbf{Tags}}      & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multirow{2}{*}{\textbf{Exact Match}} & \multirow{2}{*}{\textbf{Rationale F1}} & \multirow{2}{*}{\textbf{IOU F1}} \\
\multicolumn{1}{l}{}                                                                        & \multicolumn{1}{l}{}                     &                                     & \multicolumn{1}{c}{}                                &                                       &                                    &                                  \\ \hline
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Span\\ Prediction\end{tabular}}}         & \multirow{3}{*}{\textbf{Offensive}} & \multirow{3}{*}{B I O}          & {\fontfamily{qcr}\selectfont BERT$_{base}$}                                      & 34.9                                  & 41.9                               & 37.3                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{base}$}                                   & 34.1                                  & 40.6                               & 36.2                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{large}$}                                  & 37.8                                  & 45.4                               & \textbf{39.8}                    \\ \cline{2-8} 
                                                                                            & \multirow{3}{*}{\textbf{Target}}    & \multirow{3}{*}{B I O}          & {\fontfamily{qcr}\selectfont BERT$_{base}$}                                      & 33.5                                  & 34.1                               & 33.1                    \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{base}$}                                   & 41.1                                  & 41.9                               & 44.9                             \\
                                                                                            &                                          &                                     & {\fontfamily{qcr}\selectfont RoBERTa$_{large}$}                                  & 43.0                                  & 43.8                               & \textbf{46.4}                             \\ \bottomrule
\end{tabular}
}
\caption{Evaluation results of sentence classification and span prediction task. Experiments are done with different pretrained language models and the best results are reported. We use binary-F1 for \textit{offensive} subtask, macro-F1 for \textit{target} and \textit{group} subtask. For \textit{group} subtask, all 27 target groups are used as gold labels. \textbf{Bold} indicates the best performance across the models.}
\label{tab:baseline}
\end{table*}

==> contents/tables/context_analysis.tex <==
\begin{table}[htp]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}llrr@{}}
\toprule
                                    & \textbf{Span}  & \multicolumn{1}{l}{\textbf{Count}} & \multicolumn{1}{l}{\textbf{\%}} \\ \midrule
\multirow{2}{*}{\textbf{Offensive}} & Offensive Span & 18,422                             & 90.70                                   \\ \cmidrule(l){2-4} 
                                 & -           & 1,888 & 9.30  \\ \midrule
\multirow{2}{*}{\textbf{Target}} & Target Span & 7,788 & 43.97 \\ \cmidrule(l){2-4} 
                                 & -           & 9,926 & 56.03 \\ \bottomrule
\end{tabular}%
}
\caption{Number of comments with and without offensive/target span in the comment. "-" indicates comments without span.}
\label{tab:span}
\end{table}

==> contents/tables/offensive_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
                                                                                      & \multicolumn{3}{c}{\textbf{OFF / NOT}} & \multicolumn{3}{c}{\textbf{Offensive Span}} \\ \cline{2-7} 
\multirow{-2}{*}{\textbf{System}}                                                     & \textbf{P}   & \textbf{R}   & \textbf{F1}  & \textbf{P}   & \textbf{R}   & \textbf{F1}   \\ \hline
\begin{tabular}[c]{@{}c@{}}Seq\end{tabular}                      & 75.8         & 78.7         & 77.2         & \textbf{-}   & \textbf{-}   & \textbf{-}    \\
\begin{tabular}[c]{@{}c@{}}Span\end{tabular} & \textbf{-}   & \textbf{-}   & \textbf{-}   & 47.7         & 43.4         & 41.9          \\
\begin{tabular}[c]{@{}c@{}}Seq + Span\end{tabular}                        & 75.0         & 78.1         & 76.5         & 56.3         & 55.4         & 51.7         \\ \bottomrule
\end{tabular}
}
\caption{Evaluation results of offensiveness (OFF / NOT) and offensive span prediction. Sequence labeling model (Seq) is used for offensiveness prediction and token labeling model (Span) is used for offensive span prediction. We compare the result with multitask model (Seq + Span) trained with both labels.
}
\label{tab:multi_offensive}
\end{table}

==> contents/tables/target_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
                                  & \multicolumn{3}{c}{\textbf{Target Type}}   & \multicolumn{3}{c}{\textbf{Target Span}} \\ \cline{2-7} 
\multirow{-2}{*}{\textbf{System}} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P}  & \textbf{R}  & \textbf{F1}  \\ \hline
Seq                               & 63.6       & 58.3       & 60.3        & -  & -  & -   \\
Span       & - & - & -  & 60.2        & 67.3        & 61.9         \\
Seq + Span                         & 56.82      & 57.01      & 56.49       & 72.3        & 71.9        & 71.6        \\ \bottomrule
\end{tabular}
}
\caption{Evaluation results of target type (UNT / IND / GRP / OTH) and target span prediction using data labeled as offensive. Sequence labeling model (Seq) is used for target type prediction and token classification model (Span) is used for target span prediction. We compare the result with multitask model (Seq + Span) trained with both labels. Pretrained language model is fixed to BERT-base in this experiment.
}
\label{tab:multi_target}
\end{table}
